Quantum Extremal Islands Made Easy, PartIII: Complexity on the Brane

We examine holographic complexity in the doubly holographic model introduced in [arXiv:2006.04851][arXiv:2010.00018] to study quantum extremal islands. We focus on the holographic complexity=volume (CV) proposal for boundary subregions in the island phase. Exploiting the Fefferman-Graham expansion of the metric and other geometric quantities near the brane, we derive the leading contributions to the complexity and interpret these in terms of the generalized volume of the island derived from the induced higher-curvature gravity action on the brane. Motivated by these results, we propose a generalization of the CV proposal for higher curvature theories of gravity. Further, we provide two consistency checks of our proposal by studying Gauss-Bonnet gravity and f(R) gravity in the bulk.

==> sections/outline.tex <==
% !TEX root = ../island_complexity.tex

\rcm{Old text to be removed in the end.}\\

\rcm{I do think it is important to indicate that we are taking two things from the set up in \cite{Chen:2020uac}. First, we use the FG expansion to integrate out the bulk and produce an induced action and induced complexity on the brane. The FG expansion implies/ensures that the surfaces are extremal in the bulk (\ie away from the brane). Therefore, the second thing we must do to find the true maximum of eq.~\reef{eq:CVsubregion} is vary the profile on the brane. That means that we are effectively maximizing the brane complexity in the same spirit as eq.~\reef{eq:CVsubregion} itself.}

In this section we provide a general outline of the calculations in the next sections. In the island setup of~\cite{Chen:2020uac}, it was shown that the leading contribution to the entanglement entropy coming from the RT surface crossing the Planck \rcm{Please note that it is `Planck', not `Plank'. But let's just call it the brane, since there are no other branes in this setup.} brane can be interpreted as the Wald-Dong entropy of the induced gravity on the brane. The goal of this section is to outline a similar calculation to find the leading contributions to the holographic CV in the island phase that is a consequence of the bulk extremal volume surface crossing the Planck brane. First of all,  we start by summarizing the setup in which we will be working on. We then proceed to explain the two main ingredients in our calculation, the generalized volume and the Fefferman-Graham (FG) expansion. Combining these ingredients, we explain how to find the expansion of the (generalized) volume of the bulk surface in terms of an integral of geometric quantities over the island, which can be interpreted as the complexity of the island derived from the induced gravity action on the brane. 
%Lastly, we comment on how the extremality of the bulk extremal surface implies that the island itself is extremal in the Planck brane.


\subsection{Setup}\label{sec:setup}
\rcm{I think we will have a quick introduction to this in our introduction section.}


We will be working in a similar setup to that of~\cite{Chen:2020uac}. It consists of a doubly holographic model in the spirit of~\cite{Almheiri:2019hni}, where the Planck brane has an induced gravity action as in the Randal-Sundrum II braneworld construction~\cite{Randall:1999vf}. \rcm{We should also be referencing Karch and Randall.} We consider a $d$-dimensional holographic CFT coupled to a codimension-one conformal defect. The holographic dual corresponds of an asymptotic AdS$_{d+1}$ spacetime with a Planck brane anchored on the boundary at the conformal defect. Following the Randal-Sundrum II construction, we glue two copies of the the AdS$_{d+1}$ spacetime along the brane. The gravitational backreaction of the brane warps the bulk spacetime and effectively localizes the gravitational degrees of freedom, inducing a higher derivative gravitational action on the Planck brane. 

The setup has three equivalent descriptions, a feature of double holographic models. The \emph{bulk perspective} considers two copies of AdS$_{d+1}$ with dynamical gravity glued at a Planck brane, which is anchored at the conformal defect on the asymptotic boundary. On the \emph{brane perspective}, the holographic description of the bulk gravity in AdS$_{d+1}$ plus the brane corresponds to a holographic CFT on $S_d$ coupled to a Planck brane anchored at the conformal defect supporting dynamical gravity + the holographic CFT. Finally, the \emph{boundary perspective} consists of a holographic CFT in $S_d$ coupled to a codimension-one conformal defect. In this boundary perspective there is no dynamical gravity. For more details about the three perspectives of the setup, see section 3 of~\cite{Chen:2020uac}.

We begin by considering an asymptotically AdS$_{d+1}$ spacetime with metric
\begin{equation}\label{eq:FG}
\begin{split}
ds^2 = G_{\mu\nu} dX^\mu dX^\nu= \frac{\delta^2}{z^2} \(  dz^2 + g_{ij}(z,x^i) dx^i dx^j  \) \,, 
\end{split}
\end{equation}
\rcm{Please replace $\delta\to L$, as is standard. We can explain somewhere (in a footnote, perhaps) that working with the induced metric on the brane means the cutoff in the effective brane theory of $\tilde\delta\simeq L$.}
where $\delta$ denotes the radius of AdS$_{d+1}$ spacetime and $z$ is the radial coordinate in the bulk. Our notations in the whole paper is the following: Greek indices $\mu,\nu$ denote tensors in the bulk spacetime and run from $0$ to $d$ and Latin indices $i,j$ from the middle of the alphabet denote tensors on the codimension-1 hypersurface with fixed radial coordinate $Z$, running from $0$ to $d-1$. In these coordinates, we approach the asymptotic boundary for $z\to 0 $ and the Planck brane is located at $z=\zB \ll L$.  We focus on subregions $\mA_{\mt{L}} \cup \mA_{\mt{R}}$ which are in the island phase, meaning that the HRT surface $\cal E$ crosses the Planck brane. From the brane perspective, the entanglement entropy of the subregion $\mA_{\mt{L}} \cup \mA_{\mt{R}}$ in the island phase is decreased by adding the island contribution in the Planck brane, as per the island rule of~\cite{Almheiri:2019hni}. See figure~\ref{twoAdS} for an illustration of the island in our setup. 

The holographic complexity=volume ansatz for the reduced density matrix on a portion of the asymptotic boundary is obtained by evaluating the volume of the extremal codimension-one hypersurface ${\cal B}$ anchored at the subregion on the asymptotic boundary, as well as the HRT surface $\cal E$ in the bulk. When the brane itself contains an intrinsic gravitational theory, 
we expect that there will also be an extra contribution from the volume of the island (denoted by $V_{\rm Island}$). The construction becomes analogous to that of Dvali, Gabadadze and Porrati (DGP)~\cite{Dvali:2000hr}. When a DGP term is added to the brane, we further argue that the CV formula should include a term proportional to the volume of the island. 
Hence the CV conjecture states that the holographic complexity of subregion $\mA=\mA_{\mt{L}} \cup \mA_{\mt{R}}$ is given by 
\begin{equation}
\label{eq:CV-both}
{\cal C}_{\mt{V}}^{\rm{sub}} \(\mA_{\mt{L}} \cup \mA_{\mt{R}}\) \propto \max_{\partial {\cal B}=\mA\cup {\cal E}}   \[\frac{V\(\mB^{\rm sub}_{\mt{L}}\) + V\(\mB^{\rm sub}_{\mt{R}}\)}{\Gbulk\, \ell} + \frac{V_{\rm Island}}{\Gbrane \,\ell'}\]\,,
\end{equation}
where $\ell$ and $\ell'$ are the usual `unknown' length scales entering the CV ansatz and $\Gbrane$ is the Newton constant for the gravity theory on the brane. The quantum extremal island (denoted by $\cal I$) corresponds to the intersection of the hypersurface $\mB$ with the brane, \ie $\mB^{\rm sub}_{\mt{L}} \cap \mB^{\rm sub}_{\mt{R}}$. 

%****************************
%The volume functional is given by
%\beq\label{eq:volume}
%V({\cal B})= \int_{\cal B} d^d \xi \sqrt{h}\,.
%\eeq
%We have introduced the intrinsic coordinates $\xi^\alpha=\(z,\sigma^a\)$ for ${\cal B}$. The embedding of ${\cal B}$ is given by the functions $X^\mu = X^\mu(\xi^\alpha)$ and the induced metric $h_{\alpha\beta}$ on ${\cal B}$ is
%\beq\label{eq:h-induced}
%h_{\alpha\beta} =  \partial_\alpha X^\mu \partial_\beta X^\nu G_{\mu\nu}\,.
%\eeq
%The induced metric on the Planck brane is given by
%\beq
%\tilde{g}_{ij} = \partial_i X^\mu \partial_j X^\nu G_{\mu\nu}\,.
%\eeq
%Lastly, 
%\beq
%\tilde{h}_{ab} = \partial_a X^\mu \partial_b X^\nu G_{\mu\nu} = \partial_a \xi^\alpha \partial_b \xi^\beta h_{\alpha\beta} = \partial_a x^i \partial_b x^j \tilde{g}_{ij}
%\eeq 
%is the induced metric on the island $\cal I$. The volume of the island is
%\begin{equation}
%V\({\cal I}\) = \int_{\cal I} d^{d-1} \sigma \sqrt{\tilde{h}}\,.
%\end{equation}

The motivation of our calculation is to extract the contributions in holographic complexity ( in eq.~\eqref{eq:CV-both}) from the region around the Planck brane ( locating at $z=\zB$) and derive the leading results in terms of geometric quantities integrated over the island. Generally, the dynamic around the brane is complicated. The simplicity in our set-up originates from the special configuration with  $\zB/\delta \ll 1$. 

\subsection{Fefferman-Graham expansion}\label{sec:FG}

\rcm{This discussion needs to be kept as part of section \ref{sec:bulksubregion}.}

Around the asymptotic boundary with $z \to 0$, the Fefferman-Graham expansion provides the a series expansion of the bulk metric $g_{ij}(z,x^i)$ in terms of the ``boundary metric'' $\ov{0}{g}_{ij}$  and the ``boundary stress tensor'' $\ov{d/2}{g}_{ij}$, \ie 
\begin{equation}\label{eq:bulkexpansion}
g_{ij}( z, x^i) =  \ov{0}{g}_{ij} \( x^i \)  + \frac{z^2}{\delta^2}\ov{1}{g}_{ij} \( x^i \) + \cdots  \frac{z^d}{\delta^d} \(  \ov{d/2}g_{ij} (x^i)  + f_{ij}(x^i) \log \( \frac{z}{\delta} \)    \) \,.
\end{equation}
Near the Planck brane located at $z =\zB \ll \delta$, we can also apply the FG expansion of the metric as a natural expansion with expansion parameter $z_B/L\ll1$.

Considering the metric equations of motion near the boundary, one can fix the expansion coefficients $\ov{n}{g}_{ij}$ (with $0<n < \frac{d}{2}$) in terms of the boundary metric $ \ov{0}{g}_{ij}$. For example, the first term in the expansion is given by the Schoutten tensor $P_{ij}$ associated to the boundary metric $\ov{0}{g}_{ij}$,
\begin{equation}\label{eq:g1}
\ov{1}{g}_{ij} \( x^i \) = -L^2 P_{ij}[\ov{0}{g}] = -\frac{\delta^2}{d-2}  \( R_{ij}[\ov{0}{g}] - \frac{\ov{0}{g}_{ij} }{2(d-1)} R[\ov{0}{g}]   \) \,,
\end{equation}
where $R_{ij}$ and $R$ denotes the Ricci tensor and Ricci scalar associated with boundary metric $\ov{0}{g}_{ij}$, respectively. We further note the above expression can also be derived by examining the effect of Penrose-Brown-Henneaux (PBH) transformation, which implies the components $\ov{1}{g}_{ij} \( x^i \) $ are completely determined by the conformal symmetries on the boundary. This is why the above result is independent of the bulk gravity theory. Later, we will show that it also contributes universal terms in the holographic complexity.
The second term in the FG expansion of the metric $\ov{2}{g}_{ij}$ depends on the bulk gravity theory~\cite{Imbimbo:1999bj,Myers:2013lva}. More precisely, it depends on whether the gravitational action contains a term proportional to the Riemann tensor squared (${\cal L} \sim R_{\mu\nu\rho\sigma} R^{\mu\nu\rho\sigma}$). 

The core of the calculations in this paper consists on applying the FG expansion to different quantities in Island phase and extracting the geometric contributions associated with the island. We reinterpret (or define) those geometric contributions as the Island complexity, \ie $\mC_{\mt{V}}^{\rm Island}$. Furthermore, we find that Island complexity can also be derived from the effective action on the brane by taking account of the generalized volume term and $K$-term. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Generalized Complexity-Volume}\label{sec:gen-vol}

\rcm{I am proposing that we write out these results in the introduction.}

In this subsection, we briefly introduce the two ingredients in our proposal to the Island complexity $\mC_\mt{V}^{\rm Island}$ as well as the generalized CV for higher-curvature gravity theories. 
 %\begin{equation}
 %\mC_\mt{V}^{\rm Island} \equiv  \max_{\mI}\[ \frac{d-2}{G_{d}\ell} \( \tilde{W}_{\rm gen} (\mI)+ \tilde{W}_K(\mI) \)   \]  \,.
 %\end{equation}
\subsubsection*{Generalized Volume}
The authors of~\cite{Bueno:2016gnv} propose a generalization of the volume functional for higher derivative gravity theories. In particular, they argue that the most general local geometric functional constructed from the variation of the Lagrangian with respect to the Riemann tensor is given by the generalized volume
\begin{equation}\label{eq:defineWgen01}
W_{\rm gen}\({\cal B}\) = \int_{\cal B} d^{d}\sigma \, \sqrt{h}\,\(\alpha \frac{\partial \mathbf{L}_{d+1}}{\partial R_{\mu\nu\rho\sigma}}  n_\mu {h}_{\nu\rho} n_\sigma + \beta  \frac{\partial \mathbf{L}_{d+1}}{\partial R_{\mu\nu\rho\sigma}}  {h}_{\mu\sigma} {h}_{\nu\rho} + \gamma  \)\,,
\end{equation}
where $\mathbf{L}_{d+1}$ denotes the rescaled Lagrangian by $\mathbf{L}_{d+1}= 16\pi G_{d+1} \mathrm{L}_{d+1}$ and the timelike unit vector normal to ${\cal B}$ is $N^\mu$, \ie  $N^\mu N_\mu=-1$. 
Furthermore, $\alpha$, $\beta$ and $\gamma$ are chosen such that $W_{\rm gen}\({\cal B}\) = V\({\cal B}\)$ for Einstein gravity. Thus, it could be considered as the natural generalization for the volume element in the CV proposal to the higher-curvature gravity theory. Similarly, the generalized volume of the island $\cal I$ is given by
\begin{equation}\label{eq:defWgenI}
 \tilde{W}_{\rm gen}\({\cal I}\) = \int_{\cal I}  d^{d-1}y  \sqrt{\tilde{h}} \(   \frac{\partial \mathbf{L}_{\rm eff}}{\partial R_{ijkl}}\tilde{h}_{jk} \(  \alpha \tn_i \tn_l + \beta \tilde{h}_{il} \) + \gamma \)
\end{equation}
where $\mathbf{L}_{\rm eff}$ denotes the rescaled Lagrangian of the induced gravity on the Planck brane and $\tilde{n}^i$ is the unit vector normal to $\cal I$. 

It is obvious that one of the coefficients $\alpha$, $\beta$, and $\gamma$ is fixed by demanding that $W=V$ for Einsteing gravity. Furthermore, we find that the other two coefficients can also be fixed by matching the subleading terms in the FG expansion of  $\mC_{\mt{V}}^{\rm sub}$. In section~\ref{sec:bulksubregion}, we consider Einstein gravity in the bulk and find that these coefficients only depend on the dimension of gravity, \ie (see eq.~\eqref{eq:alphagamma})
\begin{equation}
\alpha_d = \frac{2(d-4)}{(d-2)(d-3)}\,, \quad \beta_d = 0 \,, \quad \gamma_d = \frac{2}{(d-2)(d-3)}\,.
\end{equation}

\rcm{What happens for $d=2$ and $d=3$?? Perhaps it is worth an extra subsection in section \ref{sec:bulksubregion} (or an appendix) to explain these special cases in more detail. I think it has to do with logarithms appearing either in the induced action or in the volume. Setting the logarithms aside, I am slightly worried that our conventions say that $\mC_V=0$ for $d=2$. In various discussions, people are happy to use the geodesic length in that case and I believe it shows more or less the expected behaviours as well.}

\subsubsection*{$K$-term}
The analysis in our paper is similar to other work expanding volumes of bulk hypersurfaces into integrals of geometric quantities over lower dimensional intersection of the bulk hypersurfaces with the asymptotic boundary~\cite{Hung:2011ta,Carmi:2016wjl} or with the Planck brane~\cite{Chen:2020uac}. Similar to the result in those references, the subleading terms to be integrated over the island $\cal I$ include extrinsic curvature terms, which do not appear on the original proposal for generalized volume in eqs.~\eqref{eq:defineWgen}. These extrinsic curvature terms arise from the higher-order terms $\ov{n}{x^i}$ in the FG expansion of the embedding functions, which can be seen \eg in eq.~\eqref{eq:X1}.


This situation is similar to what would occur if the results in section 4.3 of~\cite{Chen:2020uac} were attempted to be interpreted in terms of the Wald entropy~\cite{Wald:1993nt} without the intrinsic curvature corrections of~\cite{Dong:2013qoa}. Thus, inspired by generalized entanglement entropy case, we propose that the Island complexity should include a $K$-term defined by 
\begin{equation}
\tilde{W}_{K}\( \mI\)=\int_{\mI} d^{d-1}\sigma \,\sqrt{\tilde{h}}\, \frac{\partial^2 \mathbf{L}_{\rm eff}}{\partial \tR_{ijkl}\partial \tR^{mnop}} \tK_{jl}\(  A \tg_{ik} +  B \tn_i \tn_k\) \tK^{np} \( A \tg^{mo} + B \tn^m \tn^o \) \,,
\end{equation}
in addition to the generalized volume term. 

Similar to the coefficients in the generalized volume in eq.~\eqref{eq:defineWgen}, the coefficients $A$ and $B$ can be fixed by matching the subleading terms in the FG expansion of $\cal \mC_{\mt{V}}^{\rm sub}$. In section~\ref{sec:bulksubregion} with Einstein gravity in the bulk, we fix these coefficients as (see eqs.~\eqref{eq:fixB} and \eqref{eq:fixA})
\begin{equation}
A_d^2 = \frac{4(d-4)}{(d-2)^2(d-3)}\,, \quad B_d=(d-2) A_d\,.
\end{equation}
Beside the Island complexity, we also suggest to consider the generalized CV for higher-curvature gravity theories by including the generalized volume term and $K$-term. Then in section~\ref{sec:GB}, we verify that the coefficients (with dependences on the dimension) are the same for higher-curvature gravity theories in the bulk by considering Gauss-Bonnet gravity and $f(\mR)$ gravity. 

\subsubsection*{Boundary terms}
%\smr{I think this paragraph confuses the boundary term for gravity theory and the boundary term $W_{\rm bdy}$ for the generalized CV functional. It is not really right from my viewpoint. For example, the generalized CV functional from the Riemannian-square term only contain linear $R_{\mu\nu\rho\sigma}$ term. The problem is that functional can not be completely rewritten as some intrinsic quantities on the hypersurface. So the variation problem is more complicated.}

Lastly, we mention that for higher curvature gravity, extremizing the generalized CV functional $ W_{\rm gen}+W_K$ requires the addition of a boundary term $W_{\rm bdy}$ to have a well posed variational principle. For Gauss-Bonnet gravity, the bulk gravity theory is not a higher derivative theory and the boundary term $W_{\rm bdy}$ can be fixed in the same way of the
 Gibbons-Hawking term for the action of Einstein gravity. The corresponding $W_{\rm bdy}$ for Gauss-Bonnet gravity is given in eq.~\eqref{eq:GB_Wbdy}. For $f(R)$ gravity, the situation is more complicated. $f(R)$ gravity is a higher derivative term, so it has more degrees of freedom than Einstein gravity. In the case of the action, the boundary term can be fixed by considering the (classically) equivalent scalar tensor theory with action~\eqref{eq:scalartensor}. By working with the equivalent scalar tensor theory, the boundary term for generalized CV functional $W_{\rm bdy}$ simply vanishes in our analysis.



\subsection{Summary of the derivation} 
\rcm{I thought this was mostly repetitive. Perhaps some of the text can be kept as an introduction in the next section or a summary in the discussion.}


Having explained the setup and the necessary ingredients needed for the main derivation of this paper, we now summarize how the calculations in the following section go. We are interested in calculating the holographic CV for a subregion $\mA_{\mt{L}} \cup \mA_{\mt{R}}$ in the setup described in section~\ref{sec:setup} that is in the island phase. We do this first for a model with Einstein gravity in the bulk.  In section~\ref{sec:bulksubregion}, we find the identification shown in \eqref{eq:CVequalsisland} helps to fix the formulas for the generalized volume and $K$-term. Then, equipped with the proposal for generalized CV for higher-curvature gravity theories, we apply our proposals in section~\ref{sec:GB} for two higher-curvature theories in the bulk: Gauss-Bonnet gravity and $f(\mR)$ gravity.

That is, we are interested in subregions $\mA_{\mt{L}} \cup \mA_{\mt{R}}$ for which the HRT surface $\cal E$ crosses the Planck brane. Furthermore, we seek to find the leading contributions of the holographic CV due to the presence of the island $\cal I$. For this purpose, we work with a FG expansion of the metric $G_{\mu\nu}$ and the embedding functions $x^\mu$ as in eqs.~\eqref{eq:bulkexpansion} and \eqref{eqx1FG}. For each side of the asymptotically AdS bulk gravity theory,  the bulk gravitational action is given by
\begin{equation}\label{eq:Sbulk}
I_{\rm bulk} = \int_{\rm bulk} d^{d+1}X \sqrt{-G} \, {\cal L}_{\rm bulk}\[G\] + \int_{ \rm brane} d^d x \sqrt{-\tilde{g}}  \, {\cal L}_{\rm surf}[\tg,\tilde{\mK}]\,,\,,
\end{equation}
with ${\cal L}_{\rm surf}$ as the boundary term evaluated on the brane with induced metric $\tg$ and extrinsic curvature $\tilde{\mK}$, 
we derive the generalized CV functional
\begin{equation}
{\cal W}_{\rm bulk} = W_{\rm gen} + W_K+W_{\rm bdy}\,,
\end{equation}
where $W_{\rm gen}$ and $W_K$ are defined in eqs.~\eqref{eq:defineWgen} and \eqref{eq:defineWK} respectively, and the boundary term $W_{\rm bdy}$ is defined in eq.~\eqref{eq:GB_Wbdy} for Gauss-Bonnet gravity and eq.~\eqref{eq:GB_WbdyfR} for $f(R)$ gravity. There is no boundary term $W_{\rm bdy}$ for Einstein gravity. As mentioned in section~\ref{sec:gen-vol}, the generalized volume reduces to the standard volume functional if the bulk gravity action is that of Einstein gravity.

The generalized holographic CV for the boundary subregion $\mA_{\mt{L}} \cup  \mA_{\mt{R}}$ is then given by 
\begin{equation}
{\cal C}^{\rm sub}_{\mt{V}} \( \mA_{\mt{L}} \cup  \mA_{\mt{R}}  \) = \max_{\mB^{\rm sub}}  \[ \frac{(d-1)}{\Gbulk\, \ell} \(  {\cal W}_{\rm bulk}\(\mB^{\rm sub}_{\mt{L}}\) + {\cal W}_{\rm bulk}\(\mB^{\rm sub}_{\mt{R}}\)\)\]\,,
\end{equation}
where $\mB^{\rm sub}_{\mt{L}} \cup \mB^{\rm sub}_{\mt{R}}$ is the subregion of a codimension-one bulk surface which is anchored at the boundary subregion $\mA_{\mt{L}} \cup  \mA_{\mt{R}} $ and its HRT surface $\cal E$. The extremality of the generalized CV functional ${\cal W}_{\rm bulk}$ fixes the first order term in the FG expansion close to the brane as in eq.~\eqref{eq:X1} and \eqref{eq:X1GB}. Together with the FG expansion of the metric in eqs.~\eqref{eq:bulkexpansion} and \eqref{eq:g1}, we can produce an FG expansion of the holographic CV around the brane to find the leading contribution as an integral of geometric quantities over the island as in eqs.~\eqref{eq:full_subCV}, \eqref{eq:CVGBbrane02} and \eqref{eq:CVfR02}.
%\beq\label{eq:CVleading}
%{\cal C}_V = \frac{1}{\Gbulk \ell} \int_{\cal I} d^{d-1} \sigma \sqrt{\tilde{h}} \[c_0 + c_1 \tilde{R} + c_2 \tilde{R}_{ij} \tilde{n}^i \tilde{n}^j + k_1 \tilde{\cal K}^2 + k_2 \tilde{\cal K}_{ij} \tilde{\cal K}^{ij} + {\cal O} \(\frac{\zB^4}{L^4}\) \]\,,
%\eeq
%where $\tilde{R}$ and $\tilde{R}_{ij}$ are the induced Ricci scalar and tensor of the island, $\tilde{\cal K}_{ij}$ is the extrinsic curvature of the island and $\tilde{\cal K}$ its trace. The four geometric terms containing the induced curvatures and the extrinsic curvatures are ${\cal O}\(\frac{\zB^2}{L^2}\)$. The expression above corresponds to the leading contribution to the holographic CV due to the presence of the island.

In order to interpret this as the generalized CV of the island, we begin by deriving the induced gravity action on the brane 
\begin{equation}\label{eq:Sind}
I_{\rm {eff}}  = 2I_{\rm {bulk}} +  I_{\rm brane} \,.
\end{equation}
where the factor of 2 in eq.~\eqref{eq:Sind} is there to remind us that there are contributions from the bulk action at either side of the brane and $I_{\rm brane}$ denotes the intrinsic brane action
Using the FG expansion of the bulk metric $G_{\mu\nu}$ and the extrinsic curvature $\tilde{\cal K}$, we can truncate the FG expansion of the total bulk action at the leading and sub-leading orders and rewrite the induced gravitational action in terms of geometric quantities on the brane as in eqs.~\eqref{eq:effectiveaction}, \eqref{eq:actionGBbrane} and \eqref{eq:actionfRbrane}.
With the induced action associated with effective Newton constant $G_{d}$, we can derive the generalized CV functional ${\cal W}_{\rm brane} = \tilde{W}_{\rm gen} + \tilde{W}_{K}$ for the induced gravity theory on the brane. 
Finally, comparing the generalized CV derived from the gravity theory in the bulk and on the brane, we can interpret the leading terms in the holographic CV as the generalized CV of the island, \ie \eqref{eq:CVequalsisland} , with the Island complexity defined by 
\begin{equation}
\mC_\mt{V}^{\rm Island} \equiv  \max_{\mI}\[ \frac{d-2}{G_{d}\ell} \( \tilde{W}_{\rm gen} (\mI)+ \tilde{W}_K(\mI) \)   \]  \,.
\end{equation}
If the brane action contains a DGP term as in eq.~\eqref{eq:DGP}, 
then we add an island contribution to the holographic CV\footnote{\jh{If the brane action itself contained higher curvature terms, would we expect the same to hold with $V\(\cal I\)$ replaced by $\cal W\(I\)$?}\smr{I think so.}}
\begin{equation}\label{eq:CV=WB+VI}
{\cal C}_{\mt{V}}^{\rm sub} = \max_{\mB^{\rm sub}}  \[ \frac{(d-1)}{\Gbulk\, \ell} \, {\cal W}_{\rm bulk}\(\mB^{\rm sub}_{\mt{L}} \cup \mB^{\rm sub}_{\mt{R}}\) + \frac{ (d-2) }{\Gbrane \ell} V_{\rm Island}\]\,, 
\end{equation}
With the addition of the DGP term, the resulting holographic CV can also be interpreted in terms of the generalized CV of the island.
Thus due to the presence of the island, we find the leading terms in the holographic CV from bulk theory correspond to the generalized CV of the island derived from the induced gravity action on the brane. We emphasize that the equivalence as \eqref{eq:CVequalsisland} highlights the leading contribution related to the island. The UV divergences of the holographic CV are related to the the infinite proper distance to the asymptotic boundary subregion $\mA$ and consist of integrals of geometric quantities over $\mA$ as in~\cite{Carmi:2016wjl}. 
\subsection{Leftover from intro}

************************

\smr{I use $V_{\rm Island}$ for the volume of islands rather than $V(\mI)$ because we use $V(\mB)$ to present a $d$-dimensional volume.}\\

\smr{Do the following several paragraphs play the role of ``Summary of the derivation"? I only keep the minimal part for introduction for now.} 
\smr{I suggest to keep only one summary either in the introduction or in the section 2.4 .}

Similar to the bulk Einstein gravity case, the leading terms in the FG expansion of the generalized holographic CV in eq.~\eqref{eq:ourporposal} can be expanded near the brane and the leading terms correspond to the generalized volume of the island given the induced gravity action on the brane. Concretely, we are interested in computing the leading corrections to the complexity of the island by analyzing the holographic complexity of a subregion in the island phase. The leading and subleading UV divergences in the holographic CV can be recast into integrals of geometric quantities over the boundary subregion by keeping the first few terms in the FG expansion of the volume of the extremal surface $\cal B$~\cite{Carmi:2016wjl}. In a similar spirit, the leading contributions to the holographic CV due to the presence of the island can be recast as an integral of geometric quantities over the island by taking the first few terms in the FG expansion of the volume of $\cal B$, this time expanded around the intersection of $\cal B$ with the brane. The resulting expression can be recast into a similar integral over geometric quantities. The first two orders in the expansion can be interpreted as the generalized volume ${\cal W}_{\rm brane} = \tilde{W}_{\rm gen} + \tilde{W}_{K}$ of the island for the higher derivative gravity induced on the brane (see eqs.~\eqref{eq:defineWgen} and \eqref{eq:defineWK}), truncated also at second order.

This analysis can be generalized for higher derivative bulk gravity setups. In these cases, the volume of the extremal surface $\cal B$ is not enough to produce the consistent result ${\cal W}_{\rm brane} $ on the brane. The generalized CV for higher derivative gravity in the bulk is therefore given by eq.~\eqref{eq:ourporposal}
\rcm{Explicitly write out the details for our proposal for generalizing CV to a higher curvature theory.}\smr{shown in\eqref{eq:details}.}
and similarly for the subregion CV. Explicitly, we propose the holographic CV of the state defined at the asymptotic boundary subregion $\mA$ of a higher curvature bulk gravity model corresponds to the generalized volume ${\cal W}_{\rm bulk} = W_{\rm gen} + W_K$ of the bulk codimension-one surface $\cal B$ anchored at $\mA$ and its HRT surface $\cal E$. The generalized volume is derived from the bulk gravity action as in eqs.~\eqref{eq:threeW}.


\rcm{The following seems a rather detailed discussion (\ie too many equations) of our approach but I would suggest sketching the approach out in words and then leaving the equations for the next section. You should probably include the distinction between the examples that I emailed you about.}\jh{Reworked, also split the ``main results'' from the DGP discussion}


As was mentioned above, we have two main results in the present paper. First, we found that the leading contribution to the CV due to the presence of the island $\cal I$ is given by the generalized volume of the island $\tilde{W}_{\rm gen}\({\cal I}\)$ plus the intrinsic curvature term $\tilde{W}_{\tilde{K}}$ derived from the induced gravity action on the brane, see eq.~\eqref{eq:new}. Then, inspired by this result, we propose the holographic CV for higher curvature bulk gravity. The generalized CV is given by the generalized volume ${W}_{\rm gen}$ plus the K-term $W_K$ of the maximal bulk codimension-one surface $\cal B$ (plus the volume of the island $\cal I$ if there is a DGP term). This is summarized in eq.~\eqref{eq:defCV}. With this prescription, we also find that the leading contribution to the generalized holographic CV is given by the generalized CV of the island. 
%\beq\label{eq:CV-Visle}
%{\cal C}_V = \frac{d-1}{\Gbulk \ell} {\cal W}_{\rm bulk}\({\cal B}\) + \frac{d-2}{\Gbrane \ell} {V}\({\cal I}\)  \sim \frac{d-2}{G_{\rm eff} \ell} {\cal W}_{\rm brane}\({\cal I}\)\,,
%\eeq
%where ${\cal W}_{\rm bulk}$ is the generalized volume derived from the bulk gravity action, and similarly ${\cal W}_{\rm brane}$ is the generalized volume derived from the induced brane gravity action. The effective Newton's constant is given by $\frac{1}{G_{\rm eff}} = \frac{2L}{(d-2) \Gbulk} + \frac{1}{\Gbrane}$.

Lastly, we note that the extremality of the surface $\cal B$ implies that the QEI is itself an extremal surface in the brane. This is because the bulk surface $\cal B$ extremizes the generalized volume functional in the bulk $\cal W_{\rm bulk}$. The leading FG terms in the generalized volume functional correspond to the generalized volume ${\cal W}_{\rm brane}\({\cal I}\)$ of the island on the brane. Consequently, the island slice $\cal I$ is an extremal surface of the generalized volume functional $\cal W_{\rm brane}$. Since the leading term in the generalized volume is the volume of the island, this implies that the leading order term in the FG expansion of the extrinsic curvature of the island vanishes. Consequently, the terms in the generalized volume of $\cal B$ and the island that include the extrinsic curvature are of higher order than expected, and the $W_K$ only enter at higher order in the FG expansion of the CV. This result generalizes to the analyis of the entanglement entropy of the island in~\cite{Chen:2020uac}. The HRT surfaces extremize the (generalized) area functional of the bulk gravitational theory. Similar to the argument for complexity, the leading term in the (generalized) area corresponds to the Wald-Dong entropy functional. The leading term in the Wald-Dong functional is the area of the QES, which implies that the leading FG term in extrinsic curvature of the QES vanishes, and the K corrections to the Wald entropy formula are subleading.





%\begin{figure}[tb]
%	\centering\includegraphics[width=5.8in]{two_AdS.pdf}
%	\caption{Set-Up: a time slice in the $(d+1)$-dimensional bulk with two copy of AdS$_{d+1}$\label{twoAdS}}
%\end{figure}

%For example, for the case of bulk Einstein gravity studied in~\cite{Carmi:2016wjl}, the leading divergences are given by eq.~\eqref{eq:CV-carmi}.
%\beq
%\label{eq:CV-carmi}
%{\cal C}_V = \frac{L^{d-1}}{\Gbulk \delta^{d-1}} \int d^{d-1} y \sqrt{\ov{0}{\hab}} \[ \frac{1}{d-1} - \frac{\delta^2}{2(d-2)(d-3)} \( {\cal R}^a_a - \frac12 {\cal R} - \frac{(d-2)^2}{(d-1)^2}K^2\)\]\,,
%\eeq
%where $\delta$ is the UV cutoff.



